Deep Reinforcement Learning for Green Security Games with Real-Time Information

Green Security Games (GSGs) have been proposed and applied to optimize patrols conducted by law enforcement agencies in green security domains such as combating poaching, illegal logging and overfishing. However, real-time information such as footprints and agents' subsequent actions upon receiving the information, e.g., rangers following the footprints to chase the poacher, have been neglected in previous work. To fill the gap, we first propose a new game model GSG-I which augments GSGs with sequential movement and the vital element of real-time information. Second, we design a novel deep reinforcement learning-based algorithm, DeDOL, to compute a patrolling strategy that adapts to the real-time information against a best-responding attacker. DeDOL is built upon the double oracle framework and the policy-space response oracle, solving a restricted game and iteratively adding best response strategies to it through training deep Q-networks. Exploring the game structure, DeDOL uses domain-specific heuristic strategies as initial strategies and constructs several local modes for efficient and parallelized training. To our knowledge, this is the first attempt to use Deep Q-Learning for security games.

==> experiments.tex <==
\section{Experiments and Discussions}
In all of our experiments, we test our algorithms on a grid world of size $7\times 7$. The patroller always starts from the center of the map, representing the patrol post. The poacher enters the map uniformly randomly from the four corners. The poacher has 6 snares available to him in each game episode. All training and testing episodes are limited to 100 time steps. Animal densities are randomly generated numbers between 0.2 and 1.

\subsection{Baseline Defender Strategies}
We begin by describing several baseline strategies for the defender. The first two baselines are heuristic rule-based patroller and stochastic policy network. Both of them are introduced in previous sections. We employ an additional defender baseline strategy: the random sweeping strategy. Using this strategy, the defender first heads directly towards a randomly chosen edge of the map. Then, he moves along the boundary either clockwise or counterclockwise, determined at random. Empirically, this straightforward policy yields competitive performance against other baselines.

\subsection{Reactive Attacker}
First, we examine the effectiveness of different defender policies against a reactive heuristic rule-based attacker policy. The patroller is implemented with heuristic rules, policy gradient methods and deep Q-learning. The parameters $w_a$, $w_i$ and $w_o$ of the poacher's policy are set based on suggestions from domain experts. We also consider the random sweeping baseline strategy which does not require training.

When training the DQN, we use an initial learning rate of $5 \times 10^{-6}$ with decay. The learning player, in this case, the patroller, uses an epsilon-greedy policy for exploration. Since the players only have very limited local information about their opponent, the epsilon parameter is initially set to 1 and decays by 0.01 every 3000 episodes.
% (TODO: what are the values exactly? Show in a table? Response: they are chosen based on my feeling, there is no justification, so I prefer to only briefly mention this thing. I think the exact value does not matter very much.).

\begin{table}[h]
	\centering
	\begin{tabular}{c|c}
		\hline
		Patroller Model & Defender EU\\
		\hline
		Heuristic Rule-based & 2.97\\
%		\hline
		Random Sweep & 4.64 \\
%		\hline
		Stochastic Policy Network & 1.49 \\
%		\hline
		DQN & 7.23\\
		\hline
	\end{tabular}	
	\caption{Defender's expected utility (EU) against a heuristic rule-based poacher, for patrollers trained using different algorithms.}\label{tab:reactive-attacker}
%	\vspace{-10pt}
\end{table}
The defender's expected utilities are shown in Table~\ref{tab:reactive-attacker}. We observe that with a granularity of 0.1 and a searching range from -5 to +5, searching the optimal parameters for heuristic methods requires lots of simulations and can be very time-consuming. On the contrary, the DQN method can find the optimal strategy very quickly and efficiently, through the interactions between the agent and environment. The expected utility for the heuristic patroller with grid search for the optimal parameters is 2.97 and for the DQN-based patroller is 7.23, 
% (TODO: what are the optimal values of the strategy through grid search?)
from which we can tell that when faced with a non-adaptive opponent, DQN methods can effectively find a strategy that performs very well. The random sweeping strategy achieves higher performance than the grid search, while still lagging behind the results from DQN. In fact, we observe that the learned DQN strategy is a more sophisticated version of random sweeping.

\begin{figure}[h!]
	\centering
	\begin{subfigure}[b]{0.9\linewidth}
		\includegraphics[width=\linewidth]{game1}
		\caption{At timestep 22}
		\label{fig:game-1}
	\end{subfigure}%
	\\
	\begin{subfigure}[b]{0.9\linewidth}
		\includegraphics[width=\linewidth]{game2}
		\caption{At timestep 23}
		\label{fig:game-2}
	\end{subfigure}%
	\caption{Screenshots of the game, where the poacher strategy is heuristic rule based and the patroller strategy is DQN based.}\label{fig:game-screen}
%	\vspace{-15pt}
\end{figure}
On the other hand, we find that in a highly dynamic game with imperfect information like our problem, it is very difficult to effectively train a stochastic policy with policy gradient methods. One possible reason is that different from the traditional RL problems, in our game the state is only a very limited local observation and it is not informative enough to learn the optimal action distribution. Before seeing any footprints, we require the agent to perform a long sequence of random guesses and as shown in Figure \ref{fig:game-screen}, what makes DQN patroller so effective is that DQN-based patroller learns to sweep around the border until he finds any footprints to follow. While for the policy gradient methods, the optimal action distribution for any state without footprints is observed to be close to a random uniform distribution. In other words, PG methods learn an average of all possible sweeping routes, and as a result, it will be not quite effective in such a dynamic imperfect information game.
\subsection{Adaptive Attacker in Zero-Sum Games}
While the patroller can learn an effective strategy using DQN against a reactive poacher, when we train a DQN-based poacher against a fixed DQN-based patroller, we observe that the DQN-based patroller can easily be exploited by an adaptive opponent. This is because a DQN policy is a deterministic policy since given a certain state, we always choose the action with the maximum Q-value. In a security game, any pure strategy can be easily exploited by the opponent, which reveals the challenge of the proposed game. 

Nevertheless, based on the experiments above, we know that deep Q-learning can effectively approximate the best response strategy given a fixed opponent. Thus, DQN can serve as the building block for the double oracle algorithm. In this subsection, we focus on zero-sum games, where DO is guaranteed to converge to an NE (also SSE). 

\begin{table}[h]
	\centering
	\begin{tabular}{|c|c|c|}
		\hline
		Iteration $k$ & Defender EU &  Attacker EU\\
		\hline
		1 & 2.5485 & -2.5485\\
		\hline
		2 & 0.0666 &  -0.0666 \\
		\hline
		3 & -0.0912 & 0.0912 \\
		\hline
		4 & 0.4621 & -0.4621 \\
		\hline
		5 & 1.9223 & -1.9223 \\
		\hline
		Random Sweeping & 1.9245 & -1.9245 \\
\hline
	\end{tabular}
	\caption{Preliminary results of DO combined with Deep Q-learning in zero-sum games. The results shown here are when the defender uses the NE strategy computed in the restricted game of the previous iteration, and the attacker uses the best response strategy against the defender's strategy. The last row reports the results for the random sweeping baseline.}	\label{tab:zero-sum}
%	\vspace{-10pt}
\end{table}

We start with one defender strategy represented by a DQN, and learn a DQN poacher strategy against it. The starter defender DQN was learned against the heuristic poacher in the previous subsection. From there, we use our proposed deep Q-learning approach to approximate the best response strategy for each player against the NE strategy of the opponent. We test the expected utility of the defender's strategy we got from the framework against a best-responding attacker experimentally. Table~\ref{tab:zero-sum} shows the preliminary results. The second and third column shows the expected utility for the defender and attacker respectively, where the defender uses the NE strategy computed in the restricted game and the attacker uses the best response strategy against the defender's strategy (approximated by a trained DQN policy). 

Note that the best defender strategy of the first five iterations is found in iteration 1, as measured by the defender EU. It performs better than the random sweeping. It also performs worse than facing a reactive attacker, as the active attacker is now trained against it. The subsequent iterations see lower defender EU. This may be because the attacker starts to learn smarter strategies which undermines defender strategy in iteration 1. We observe that by iteration 5, the defender has adapted to the attacker, and has learned a quite effective mixed strategy. 

We also observe that DO has not converged within five iterations, as expected. In fact, the values fluctuate a lot, leading to the concern that limiting the number of iterations in DO may be at the cost of solution quality.



\subsection{Adaptive Attacker in General-Sum Games}
In this subsection, we further investigate the performance of our framework in general-sum games. We lose the theoretical guarantee with DO in general-sum games. However, as we now show below, our framework still achieves promising empirical results.


% The third column shows when the defender's expected utility when he uses the NE strategy in the restricted game but the attacker is best responding (approximated by trained DQN policy). 
%Our first observation is that the absolute values in the two columns are positively correlated. This means this framework is promising for complex Stackelberg Security games that are near-zero-sum.
%Our first observation is that the absolute values in the second and third column are similar. This means this framework is promising for complex Stackelberg Security games that are near-zero-sum. 
The results are summarized in Table~\ref{tab:general-sum}. The first observation is that the best defender strategy of the first five iterations is found in iteration 4. The solution quality in iteration 4 is much higher than the first iteration as well as the random sweeping baseline. This suggests using double oracle with deep Q-learning can be a promising way to find a good mixed strategy for the defender for such a complex game setting. 

Similar to the experiments with zero-sum games, the values fluctuate a lot across iterations. To compensate for the loss in solution quality by the early termination of DO, we apply the evolution strategies on the outputs of DO. Fixing the DQN parameters, we iteratively update the patroller's and the poacher's mixed strategy using ES. After over 1500 iterations of ES, we, again, use deep Q-learning to find the poacher's best response to the new defender's mixed strategy. As shown in Table~\ref{tab:general-sum}, ES improves the defender EU from 2.1703 to 3.0718, effectively boosting the solution quality. Therefore, ES can be a good heuristic to post-process the potentially suboptimal solution by stopping DO prematurely.
\begin{table}
	\centering
	\begin{tabular}{|c|c|c|}
		\hline
		Iteration $k$ & Defender EU &  Attacker EU\\
		\hline
		1 & 1.2704 & 1.3151\\
		\hline
		2 & 2.454 &  1.1046 \\
		\hline
		3 & 2.815 & 0.4727 \\
		\hline
		4 & 3.6981 & 0.1007 \\
		\hline
		5 & 2.1703 & 0.6831 \\
		\hline
		After ES & 3.0718 & 0.3300 \\
		\hline
		Random Sweeping & 3.1054 & -0.2325 \\
\hline
	\end{tabular}
	\caption{Similar experiment as in Table~\ref{tab:zero-sum} for general-sum games. The ES row represents the results from performing ES on the mixed strategies from 5 iterations. The last row reports the results for the untrained baseline random sweeping.}	\label{tab:general-sum}
%	\vspace{-10pt}
\end{table}
%First, we want to examine the effectiveness of different defender policies against a reactive heuristic rule-based attacker policy. In the first set of experiments, the patroller is implemented with heuristic rules, policy gradient methods and deep Q-learning and fight against a fixed heuristic poacher, whose parameters $w_a$, $w_i$ and $w_o$ are set based on suggestions from domain experts.
%% (TODO: what are the values exactly? Show in a table? Response: they are chosen based on my feeling, there is no justification, so I prefer to only briefly mention this thing. I think the exact value does not matter very much.).
%
%\begin{figure}[t]
%\centering
%\begin{subfigure}[b]{0.7\linewidth}
%                \includegraphics[width=\linewidth]{game1}
%                \caption{At timestep 22}
%                \label{fig:game-1}
%\end{subfigure}%
%\\
%\begin{subfigure}[b]{0.7\linewidth}
%                \includegraphics[width=\linewidth]{game2}
%                \caption{At timestep 23}
%                \label{fig:game-2}
%\end{subfigure}%
%\caption{Screenshots of the game, where the poacher strategy is heuristic rule based and the patroller strategy is DQN based.}\label{fig:game-screen}
%\vspace{-15pt}
%\end{figure}
%
%In the experiments, we observe that with a granularity of 0.1 and searching range from -5 to +5, searching optimal parameters for heuristic methods requires lots of simulations and can be very time-consuming. On the contrary, DQN methods can find the optimal strategy very quickly and efficiently, through the interactions between the agent and environment. The expected utility for the heuristic patroller with grid search for the optimal parameters is 2.97 and for the DQN-based patroller is 7.23, 
%% (TODO: what are the optimal values of the strategy through grid search?)
%from which we can tell that when faced with a non-adaptive opponent, DQN methods can effectively find a strategy that performs very well. 

\iffalse
Then a natural solution should be that instead of learning an action-value function and taking actions greedily, we can directly optimize a stochastic policy. However, in our experiments, we find that in such a highly dynamic game with imperfect information, it is very difficult to effectively train a stochastic policy with policy gradient methods. One possible reason is that different from the traditional RL problems, in this game the state is only a very limited local observation and it is not informative enough to learn the optimal action distribution. Before seeing any footprints, we require the agent to perform a long sequence of random guesses and as shown in Figure \ref{fig:game-screen}, what makes DQN patroller so effective is that DQN-based patroller learns to sweep around the border until he finds any footprints to follow. While for the policy gradient methods, the optimal action distribution for any state without footprints is observed to be close to a random uniform distribution. In other words, PG methods learn an average of all possible sweeping routes, and as a result, it will be not quite effective in such a dynamic imperfect information game.
\fi
%Based on the above experiment, we know that DQN is good at approximating the best response strategy given a fixed opponent. But we also aim to find the optimal defender strategy in a Stackelberg setting. As mentioned previously, one possible way of computing Nash Equilibrium in such a game is using Double Oracle algorithm \cite{mcmahan2003planning,jain2011double,jain2013security}. When the game is zero-sum, the NE strategy is also the SSE strategy for the defender. If we treat a DQN policy as a pure strategy, then essentially we want to find the optimal mixed strategy over a pool of DQN pure strategies. Specifically, we can start with a small set of initial DQN policies for both players, and at each iteration, we first get the payoff matrix for current pure strategies with simulations and compute the Nash Equilibrium for the current game matrix. Then we fix the mixed strategy for one player and compute the best response strategy of another player with deep Q-learning. After getting a new best response policy for each player, we evaluate the value of the new payoff matrix and repeat the procedure until convergence. Even if the game is not zero-sum, but the two players' payoffs are negatively correlated (as in our setting), we hypothesize the DO algorithm which approximates NE strategy may still provide a good strategy for the defender assuming the attacker is best-responding. We, therefore, adopt the DO framework and use DQN to approximate the best response strategy for each player, and test the expected utility of the defender's strategy against a best-responding attacker experimentally. Table \ref{table} shows the preliminary results. The second and third column shows the expected utility for the defender and attacker respectively, where the defender uses the NE strategy in the restricted game (obtained in iteration $k$) and the attacker uses the best response strategy (approximated by trained DQN policy in iteration $k+1$). 
%% The third column shows when the defender's expected utility when he uses the NE strategy in the restricted game but the attacker is best responding (approximated by trained DQN policy). 
%Our first observation is that the absolute values in the two columns are positively correlated. This means this framework is promising for complex Stackelberg Security games that are near-zero-sum.
%%Our first observation is that the absolute values in the second and third column are similar. This means this framework is promising for complex Stackelberg Security games that are near-zero-sum. 
%The second observation is that the best defender strategy of the first four iterations is found in iteration 3, as measured by the value in the third column, and the solution quality is much higher than the first iteration where the defender is using an optimal deterministic strategy against a fixed opponent. This means using double oracle can effectively find a better mixed strategy for the defender compared to the deterministic defender strategy trained against the fixed opponent. Our third observation is that double oracle has not converged within four iterations, which is as expected, but also shows that limiting the number of iterations in Double Oracle to be small may lead to concerns in the resulting solution quality.
%\begin{table}[t]
%\centering
%\caption{Preliminary results of double oracle algorithm combined with DQN to approximate the best response strategy for each player. The Expected Utilities (EU) in the table are the simulation results when the defender uses the NE strategy (obtained in iteration $k$) and the attacker uses the best response strategy (approximated by DQN in iteration $k+1$).}
%\label{table}
%\begin{tabular}{|c|c|c|}
%\hline
%Iteration $k$ & Defender-NE EU &  Attacker-BR EU\\
%\hline
% 1 & -5.8775 & 5.9038\\
%\hline
% 2 & -4.3308 &  5.1455 \\
%\hline
% 3 & -1.8848 & 2.6240 \\
%\hline
% 4 & -3.7824 & 3.9441 \\
%\hline
%\end{tabular}
%\vspace{-10pt}
%\end{table}



==> future_directions.tex <==
\section{Future Research Directions}
Since training a best response DQN policy against the new opponent is often time-consuming, we can only run double oracle algorithm for a few iterations given limited computation resources and training time. Even with the DCH framework proposed by \cite{lanctot2017unified}, the limited number of iterations still present as a major bottleneck. This is one major challenge for future research. 

Also, we argue that the key online information and timing aspects should not be neglected by the security game community. Integrating deep reinforcement learning with classical game-theoretic approaches can be a promising way of finding solutions to such complex problems. Alternative frameworks need to be proposed to find SSEs instead of NEs efficiently when the game is not near zero-sum.

%In this section, we provide some promising research directions of combining traditional game-theoretic solutions with deep reinforcement learning for solving the imperfect-information security game with online interactions and finding the SSE strategy of the defender.

%Based on the above discussion, we know that DQN is good at finding the best response strategy given a fixed opponent. As mentioned previously, one possible way of computing Nash Equilibrium in such a game is using Double Oracle algorithm \cite{mcmahan2003planning,jain2011double,jain2013security}. If we treat a DQN policy as a pure strategy, then essentially we want to find the optimal mixed strategy over a pool of DQN pure strategies. Specifically, we can start with a small set of initial DQN policies for both players, and at each iteration, we first get the payoff matrix for current pure strategies with simulations and compute the Nash Equilibrium for the current game matrix. Then we fix the mixed strategy for one player and compute the best response strategy of another player with deep Q-learning. After getting a new best response policy for each player, we evaluate the value of the new payoff matrix and repeat the procedure until convergence. 

%However, training a best response DQN policy against the new opponent is often time-consuming, which results in that we can only run double oracle algorithm for a few iterations given limited computation resources and training time. To address this issue, we propose to use meta-learning algorithms \cite{finn2017model,al2017continuous} for quickly adapting to the new opponent and getting the best response policy. The rationale is that, from the perspective of feature learning, the low-level layers of a deep neural network learns to build an internal representations that can be widely suitable for many consecutive tasks. For example, any best response policy requires a good intermediate level representation of the raw input features, such as footprints and animal density, which is transferrable across different iterations.
%This indicates that after appropriately initializing the parameters of a new policy network, we can fine-tune the parameters of the high-level layers, to enable the model to quickly adapt to new opponent strategies. 
% And intuitively, we suppose that a simple way to get a reasonable initialization is to use an average of the parameters of the history policies.

%Since no previous mathematical programming based methods are applicable for such a complex game; we believe that this is a promising solution for computing Nash Equilibrium in the proposed game. Most importantly, we argue that the key online information and timing aspects should not be neglected by the security game community and deep reinforcement learning could be a powerful method to address such issues.

% \section{Related Work and Conclusion}
% (TODO: We don't need to do it for this paper, but will need it for a conference submission. We will need to discuss patrolling games, security games that can be modeled as stochastic games, other games with online information, e.g., poker)
% \newpage

==> part2.tex <==
\section{Optimal Defender Strategy Against Reactive Attacker}
In this section, we consider the case where the attacker is reactive and find the optimal defender strategies. Before discussing the computation of equilibrium strategies, we first consider how to efficiently represent a player's pure or mixed strategies.
Given the complexity of the game, finding the optimal policy is challenging. In fact, the memory needed for just representing a player's pure strategy in the form of a detailed mapping from full observation and action history to action grows exponentially in the size of the game. Therefore, representing a player's mixed strategy in its naive form (a probability distribution over the pure strategies) can be intractable.
Therefore, we consider several compact representations of the pure or mixed strategy using the key elements of the history and the environment and look for the defender's optimal strategy in the restricted space. 

%We focus on the neural network based policy and propose to use deep reinforcement learning based algorithms to find the empirical optimal defender strategy against a reactive attacker with known parameters\footnote{For heuristic rule-based policy, we simply use grid search to find the parameters of the empirically optimal defender strategy in the restricted space.}.


\subsection{Boundedly Rational Poacher Behavioral Model: The heuristic rule based non-adaptive poacher}
The poacher's policy is two-fold. At each time step, he should decide whether to put a snare at the current location and which direction to move along. First, we consider the movement decision.

Suppose the current coordinate of the poacher is $(m,n)$ and the maximum coordinate on the map is $(M,N)$. We can define the average animal density for the \emph{up} direction as $\frac{1}{(m-1)\cdot N} \sum_{0 \leq i<m, 0 \leq j \leq N} \mathcal{A}_{i,j}$, where $\mathcal{A}_{i,j}$ is the animal density for area with coordinate $(i,j)$. Similarly, we can define the average animal density for all the other directions. For simplicity, we will use an integer $k \in \{1,\ldots,5\}$ to denote one of the five directions (the fifth ``direction'' is for the action ``stand still''). This way, we can get an average animal density vector $A \in \mathbb{R^+}^5$ ($A_5$ is the animal density of the current location). 
Another important factor that should be taken into consideration is the observed footprints. We use vectors $I \in \{0,1\}^5$ and $O \in \{0,1\}^5$ to represent the footprints states, where each dimension $I_k$ (or $O_k$) is a binary variable, indicating whether or not there is an entering (or leaving) footprint from that direction (for the fifth ``stand still'' direction, $I_5 = O_5 = 0$). Now we can define the heuristic policy for poacher's movement as
\begin{equation}
\pi_{po}(a^{po}_t = k|s^{po}_t) = \frac{\exp(w_a \cdot A_k + w_i \cdot I_k + w_o \cdot O_k)}{\sum_{z} \exp(w_a \cdot A_z + w_i \cdot I_z + w_o \cdot O_z)}
\end{equation}
where $w_a$, $w_i$ and $w_o$ are parameters for the average animal density, enter footprints and leaving footprints respectively. 

% When faced with a fixed opponent, we use parameter search to find the empirically optimal strategy in this model family.\lantao{Even with the same time, this method is not necessarily comparable to DQN, since it can only represent a simple linear weighted combination of different factors, i.e., the capacity of the model family is not enough.}

Since a higher animal density means a higher probability of catching an animal, we define the probability of placing a snare in grid $(m,n)$ as
\begin{equation}
\sigma_{po}(b^{po}_t = 1|s^{po}_t) = \frac{\exp(A_{m,n} / \tau)}{\sum_i\sum_j \exp(A_{i,j} / \tau)},
\end{equation}
where $\tau$ is a temperature parameter. 

The poacher's behavioral model $(\pi_{po}, \sigma_{po})$ as described above is boundedly rational. The poacher does not adapt his strategy to the patroller's strategies, and hence does not necessarily carries out the best response. Real-world applications often feature bounded rationality due to subjective or objective constraints. Therefore, our model does apply to a wide range of problems.
% Again we can use parameter search to find the empirically optimal solution.

%Like the defender's policy, we can use a similar convolutional neural network structure to represent the attacker's strategy. The only difference is that we should change the output layer since the action space combines both the movement decisions and placing snare decisions.



\subsection{Defender Policy Representation: Q-network}
%We aim to find the defender's optimal (mixed) policy.
We may use a similar, and even simpler, heuristic policy for the defender, as the defender's decision only involves movement\footnote{For this heuristic rule-based policy, we simply use grid search to find the parameters of the empirically optimal defender strategy in the restricted space.}. Instead, we propose to represent the defender policy by a neural network, and use reinforcement learning to find an empirically optimal strategy. From the perspective of RL, at each time step $t$, the state of the patroller $s^{pa}_t$ comprise his memory of the opponent's observed footprints, current position coordinates, the corresponding terrain information, i.e., animal density and the normalized game time. The policy $\pi_{pa}(a^{pa}_t|s^{pa}_t)$ for the patroller is a mapping from his state space to his action space.

% the state of the poacher $s^{po}_t$ and patroller $s^{pa}_t$ comprise their memory of the opponent's observed footprints, current position coordinates, the corresponding terrain information, i.e., animal density and the normalized game time. 
% (TODO: not clear. Need more explanation. Current position coordinates are normalized as a scalar input? Or a binary matrix? Terrain information for all the cells in the grid? What does ``time and memory for footprint'' mean? Time is a scalar input? Memory of footprints is represented by 10 binary matrix, one for \{each direction\} x \{entering or leaving\}? Or 10 matrix for each time step?) 
% The policy $\pi_{pa}(a^{pa}_t|s^{pa}_t)$ and $\pi_{po}(a^{po}_t|s^{po}_t)$ for the patroller and poacher respectively will be a mapping from their state space to their action space.

Since the game state has strong spatial patterns, here we employ a convolutional neural network (CNN) for implementing the learning policy. The CNN takes as input a 3-D tensor, with the same width and height as the grid world and each channel representing different features. Specifically, the first eight channels are binary values indicating the existence of each kind of footprints (\{four directions\} $\times$ \{entering or leaving\}); the ninth channel is the animal density; the tenth channel is one-of-K encoding, indicating the agent's current location; the eleventh channel is the normalized time step, which is the same for all grids.
% (TODO: which ones? terrain and footprint?). 
In our experiments, the defender neural network takes a state representation of size $7 \times 7$ as input. The first hidden layer is a convolutional layer with 16 filters of size $4 \times 4$ and strides $1 \times 1$. The second layer is a convolutional layer with 32 filters of size $2 \times 2$ and strides $2 \times 2$. Each hidden layer is followed by a $relu$ non-linear transformation and a max-pooling layer. The output layer is a fully-connected dense layer which transforms the hidden representation of the state to the final policy. If the neural network is an action-value network, then each output dimension represents the Q-value for each action. The neural network corresponds to a pure strategy for the defender where the defender takes the action with the highest Q-value generated by the network, with the given state as input. If the neural network is a stochastic policy network, then each output dimension represents the probability of an action $\pi_{pa}(a^{pa}_t|s^{pa}_t)$. The neural network then corresponds to a mixed strategy for the defender where the probability of taking each pure strategy is the joint probability of taking the chosen action in each time step.

While some pure or mixed defender strategies cannot be captured by the neural network based representation, the strong expressiveness makes it a memory-efficient alternative. Furthermore, as detailed in later sections, the NN-based representation combined with RL algorithms leads to defender strategies that perform well empirically. And we expect that the current feedforward neural network implementation of the policy can further be strengthed by incorporating recurrent neural networks, such as Long Short-Term Memory networks \cite{hausknecht2015deep}.

% While this compact representation still leads to a loss in the solution quality compared to the optimal solution; we expect the empirically optimal strategy found in the restricted space is close to the optimal solution given the strong expressiveness of the representation, which can further

\subsection{Defender Policy Training: Double DQN}
With deep reinforcement learning, the intelligence of the agent can evolve through the interactions between the agent and the environment. Generally, there are two categories of RL methods, i.e. the value based methods and the policy based methods. 
% \lantao{In general, value-based methods also include learning state-value function, like AlphaGo. Q-learning is the most straightforward and widely-used one, which learns the action-value.} 
For value based methods, one of the most effective and efficient methods is Deep Q-Learning~\cite{mnih2015human}, which uses an off-policy replay buffer to keep all the transitions $(s_t, a_t, r_t, s_{t+1})$ and update the deep Q-network (DQN) as
\begin{equation}
Q(s_t,a_t) \leftarrow r_t + \gamma \max_{a'} Q^{\text{target}}(s_{t+1}, a')
\end{equation}
To solve the proposed game, which involves a highly dynamic environment, we employ the double DQN methods \cite{van2016deep} to improve the stability of training:
\begin{equation}
Q(s_t,a_t) \leftarrow r_t + \gamma Q^{\text{target}}(s_{t+1}, \arg\max_{a'} Q(s_{t+1}, a'))
\end{equation}
For policy based methods, i.e., the stochastic policy representation, we directly optimize the $\theta$-parametrized policy with the policy gradient theorem \cite{sutton2000policy}
\begin{align}
	\nabla_\theta \mathbb{E}_\tau [R] &= \mathbb{E}_\tau [\sum_{t=0}^T \nabla_\theta \log \pi(a_t|s_t,\theta) \cdot (Q^\pi(s_t, a_t) - V^\pi(s_t))]\nonumber\\ 
	&= \mathbb{E}_\tau [\sum_{t=0}^T \nabla_\theta \log \pi(a_t|s_t,\theta) \cdot A^\pi(s_t,a_t)]
\end{align}
where the advantage function $A^\pi(s_t,a_t)$ can either be approximated by Monte Carlo methods or neural networks. In our experiments, for a lower variance, we use a neural network to approximate the state-value function $V^\pi(s)$, and use $r(s_t,a_t) + V^\pi(s_{t+1}) - V^\pi(s_t)$ as an unbiased estimation of the advantage function $A^\pi(s_t,a_t)$, i.e. the actor-critic algorithm \cite{konda2000actor}.
